Programming Language Case Studies Can Be Deep

In the pedagogy of programming languages, one well-known course structure is to tour multiple languages as a means of touring paradigms. This tour-of-paradigms approach has long received criticism as lacking depth, distracting students from foundational issues in language theory and implementation. This paper argues for disentangling the idea of a tour-of-languages from the tour-of-paradigms. We make this argument by presenting, in depth, a series of case studies included in the Human-Centered Programming Languages curriculum. In this curriculum, case studies become deep, serving to tour the different intellectual foundations through which a scholar can approach programming languages, which one could call the tour-of-humans. In particular, the design aspect of programming languages has much to learn from the social sciences and humanities, yet these intellectual foundations would yield far fewer deep contributions if we did not permit them to employ case studies.

==> eptcsdata.tex <==
\providecommand{\firstpage}{56}
\providecommand{\publicationstatus}{Stephen Chang (Ed.): Trends in Functional\\ Programming in Education (TFPIE)
\\
EPTCS 405, 2024, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.405.4}{10.4204/EPTCS.405.4}}
\pdfoutput=1

